Good-for-Game QPTL: An Alternating Hodges Semantics

An extension of QPTL is considered where functional dependencies among the quantified variables can be restricted in such a way that their current values are independent of the future values of the other variables. This restriction is tightly connected to the notion of behavioral strategies in game-theory and allows the resulting logic to naturally express game-theoretic concepts. The fragment where only restricted quantifications are considered, called behavioral quantifications, can be decided, for both model checking and satisfiability, in 2ExpTime and is expressively equivalent to QPTL, though significantly less succinct.

==> Acknowledgments.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Acknowledgments.tex                                                        %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Acknowledgments.tex

\begin{section}*{Acknowledgments}

  Partially supported by the GNCS 2020 project ``Ragionamento Strategico e
  Sintesi Automatica di Sistemi Multi-Agente''.

\end{section}

% End of file Acknowledgments.tex


==> Algorithms.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Algorithms.tex                                                             %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Algorithms.tex

%%****************************************************************************%%
%% Required packages                                                          %%
%%****************************************************************************%%

\usepackage[ruled,vlined]{algorithm2e}

%%****************************************************************************%%

%%****************************************************************************%%
%% Basic settings                                                             %%
%%****************************************************************************%%

\DontPrintSemicolon

\SetKw{Signature}{signature}
\SetKwFor{Function}{function}{}{}
\SetKwFor{Procedure}{procedure}{}{}

\SetKwFor{Let}{let}{in}{}

%%****************************************************************************%%

%%****************************************************************************%%
%% Algorithms                                                                 %%
%%****************************************************************************%%

\AfterEndPreamble
  {

  %%**************************************************************************%%

  }

%%****************************************************************************%%

% End of file Algorithms.tex


==> Conclusion.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Conclusion.tex                                                             %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Conclusion.tex

\begin{section}{Conclusion}

  \cbstart
  ...
  \cbend

\end{section}

% End of file Conclusion.tex


==> Preliminaries.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Preliminaries.tex                                                          %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 2020, Dylan Bellier, Massimo Benerecetti, Dario Della Monica,%%
%%                     and Fabio Mogavero.                                    %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Preliminaries.tex

\begin{section}{Preliminaries}
  \label{sec:prl}

  \cbstart
  ...
  \cbend

  A two-player turn-based \emph{arena} $\Arena = \tuple {\PPosSet} {\OPosSet}
  {\iposElm} {\MovRel}$ is a tuple where
  \begin{inparaenum}
    \item
      $\PPosSet$ and $\OPosSet$ are the sets of \emph{positions} of
      \emph{Eloise} and \emph{Abelard}, \aka \emph{Player} and \emph{Opponent},
      respectively, with $\PPosSet \cap \OPosSet = \emptyset$,
    \item
      $\iposElm \in \PosSet \defeq \PPosSet \cup \OPosSet$ is the \emph{initial
      position}, and
    \item
      $\MovRel \subseteq \PosSet \times \PosSet$ is the binary relation
      describing all possible \emph{moves} such that $\tuple{\PosSet}{\MovRel}$
      is a sinkless directed graph.
  \end{inparaenum}

  A \emph{path} $\pthElm \!\in\! \PthSet \!\subseteq\! \PosSet[][\infty]$ is a
  finite or infinite sequence of positions compatible with the move relation,
  \ie, $((\pthElm)_{i}, (\pthElm)_{i + 1}) \in \MovRel$, for all $i \in
  \numco{0}{\card{\pthElm} - 1}$; it is \emph{initial} if $\card{\pthElm} > 0$
  and $\fst{\pthElm} = \iposElm$.
  %
  A \emph{history} for player $\alpha \in \{ \PlrSym, \OppSym \}$ is a finite
  initial path $\hstElm \in \HstSet[\alpha] \subseteq \PthSet \cap (\PosSet[][*]
  \cdot \PosSet[\alpha])$ terminating in an $\alpha$-position.
  %
  A \emph{play} $\playElm \in \PlaySet \subseteq \PthSet \cap \PosSet[][\omega]$
  is just an infinite initial path.

  A \emph{strategy} for player $\alpha \in \{ \PlrSym, \OppSym \}$ is a function
  $\strElm[\alpha] \in \StrSet[\alpha] \subseteq \HstSet[\alpha] \to \PosSet$
  mapping each $\alpha$-history $\hstElm \in \HstSet[\alpha]$ to a position
  $\strElm[\alpha](\hstElm) \in \PosSet$ compatible with the move relation, \ie,
  $(\lst{\hstElm}, \allowbreak \strElm[\alpha](\hstElm)) \in \MovRel$.
  %
  A path $\pthElm \in \PthSet$ is \emph{compatible} with a pair of strategies
  $(\pstrElm, \ostrElm) \in \PStrSet \times \OStrSet$ if, for all $i \in
  \numco{0}{\card{\pthElm} - 1}$, it holds that $(\pthElm)_{i + 1} =
  \pstrElm((\pthElm)_{\leq i})$, if $(\pthElm)_{i} \in \PPosSet$, and
  $(\pthElm)_{i + 1} = \ostrElm((\pthElm)_{\leq i})$, otherwise.
  %
  The \emph{play function} $\playFun \colon \PStrSet \times \OStrSet \to
  \PlaySet$ returns, for each pair of strategies $(\pstrElm, \ostrElm) \in
  \PStrSet \times \OStrSet$, the unique play $\playFun(\pstrElm, \ostrElm) \in
  \PlaySet$ compatible with them.

  A \emph{game} $\Game = \tuple {\Arena} {\ObsSet} {\WinSet}$ is a tuple where
  $\Arena$ is an arena, $\ObsSet \subseteq \PosSet$ is the set of
  \emph{observable positions}, and $\WinSet \subseteq \ObsSet^{\omega}$ is the
  set of \emph{observable sequences} that are \emph{winning} for Eloise; the
  complement $\dual{\WinSet} \defeq \ObsSet^{\omega} \setminus \WinSet$ is
  \emph{winning} for Abelard.

  ... \FM{To introduce parity games.}

  The \emph{observation function} $\obsFun \colon \PthSet \to \ObsSet[][\infty]$
  associates with each path $\pthElm \in \PthSet$ the ordered sequence $\wElm
  \defeq \obsFun(\pthElm) \in \ObsSet[][\infty]$ of all observable positions
  occurring in it; formally, there exists a monotone bijection $\fFun \colon
  \numco{0}{\card{\wElm}} \!\to\! \set{\! j \!\in\! \numco{0}{\card{\pthElm}} }{
  (\pthElm)_{j} \!\in\! \ObsSet \!}$ satisfying the equality $(\wElm)_{i} =
  (\pthElm)_{\fFun(i)}$, for all $i \in \numco{0}{\card{\wElm}}$.

  ... \FM{To recall that we are only considering perfect-information games, even
  if the winning condition is defined on some of the positions.}

  Eloise \emph{wins} the game if there exists a strategy $\pstrElm \in \PStrSet$
  such that $\obsFun(\playFun(\pstrElm, \ostrElm)) \in \WinSet$, for all
  $\ostrElm \in \OStrSet$.
  Similarly, Abelard \emph{wins} the game if there exists a strategy $\ostrElm
  \in \OStrSet$ such that $\obsFun(\playFun(\pstrElm, \ostrElm)) \in
  \dual{\WinSet}$, for all $\pstrElm \in \PStrSet$.
  %
  Recall that, thanks to Martin's determinacy theorem~\cite{Mar75,Mar85}, all
  Borelian games are determined, \ie, when the winning condition $\WinSet$ is a
  Borel set in the Cantor topological space of infinite words~\cite{PP04},
  either one of the two players necessarily wins the game.

  \cbstart
  ...
  \cbend

\end{section}

% End of file Preliminaries.tex


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Article"
%%% End:


==> SectionIIIa.tex <==

\subsection{Normalizing Quantifiers}

Consider two sentences $\phi \defeq \forall^{\BSym} \apElm \ldotp
\exists^{\SSym} \qapElm \ldotp \psi$ and $\varphi \defeq \exists^{\BSym} \qapElm
\ldotp \forall^{\BSym} \apElm \ldotp \psi$, similar to those used in
Example~\ref{exm:bhcsat}.
One can show that they are equisatisfiable by following the intuition developed
below.

\cbstart
Let us follows Hintikka's game-theoretic interpretation of the quantifiers for
the two formulae.
At each round $k$ of the game for $\phi$, Abelard, when choosing the value for
$\apElm$, can only read the past values chosen by Eloise for $\qapElm$ up to
round $k - 1$, since he moves first.
Eloise, instead, when choosing $\qapElm$ is forced to read the values for
$\apElm$ up to round $k-1$, since the quantification is strongly behavioral.
Thus, even if she moves second, has no knowledge about the current move of her
adversary.
Conversely, at each round $k$ of the game for $\varphi$, when choosing the value
for $\qapElm$, Eloise can only read the past values chosen by Abelard for
$\apElm$ up to round $k - 1$.
Abelard, instead, when choosing $\apElm$, can read the values for $\qapElm$ up
to round $k$ included.

Suppose that $\phi$ is satisfiable.
This means that Eloise can win the game for $\phi$ without knowing, at each
round $k$, the value of $\apElm$ at that round.
But then she can make the exact same choices and win the game for $\varphi$,
where she moves first and cannot read the choices of Abelard at round $k$
either.
%
For the other direction, assume $\phi$ unsatisfiable.
This means that Abelard wins the game for $\phi$ and he does so knowing, at each
round $k$, only to the choices of Eloise up to round $k - 1$.
He can then ignore, at each round $k$ of the game for $\varphi$, the additional
information on the value of $\qapElm$ and use the same exact choices as in the
previous game for $\phi$, which proves $\varphi$ unsatisfiable as well.
%
A symmetric argument allows to show that $\phi \defeq \exists^{\BSym} \qapElm
\ldotp \forall^{\SSym} \apElm \ldotp \psi$ and $\varphi \defeq \forall^{\BSym}
\apElm \ldotp \exists^{\BSym} \qapElm \ldotp \psi$ are equisatisfiable as well.
\cbend

The two examples above witness a general phenomenon that allows to swap two
adjacent dual behavioral quantifiers at the cost of restricting one of the two
to be strongly behavioral \wrt the proposition of the other one.
By iteratively swapping adjacent quantifiers and adjusting the quantifier
specification accordingly, we can reduce the quantifiers alternations to at most
one, while preserving satisfiability.
This idea is at the basis of the two normal forms defined below.

For technical convenience we use a vector notation for the quantifier prefixes:
$\Qnt^{\vec{\spcElm}} \vec{\apElm} \ldotp \phi \defeq \Qnt^{(\vec{\spcElm})_{0}}
(\vec{\apElm})_{0} \ldotp \cdots \Qnt^{(\vec{\spcElm})_{k}} (\vec{\apElm})_{k}
\ldotp \phi$, where $\card{\vec{\apElm}} = \card{\vec{\spcElm}} = k + 1$.
We omit the vector symbol in $\vec{\spcElm}$ if this is just a sequence of
$\BSym$ or $\SSym$ specifications and consider $\vec{\apElm}$ as sets of
propositions when convenient.
We also define the union of two quantifier specifications naturally as follows:
\begin{center}
  $\dep{ \PSet[\BSym 1] }{ \PSet[\SSym 1] } \cup \dep{ \PSet[\BSym 2] }{
  \PSet[\SSym 2] } \defeq \dep{ \PSet[\BSym 1] \cup \PSet[\BSym 2] }{
  \PSet[\SSym 1] \cup \PSet[\SSym 2] }$.
\end{center}

We now introduce the two syntactic transformations $\CSym[\QEA](\cdot)$ and
$\CSym[\QAE](\cdot)$ that, given an arbitrary behavioral quantifier prefix
$\qntElm \in \QntSet[\BSym]$, return the single-alternation ones
$\CSym[\QEA](\qntElm)$ and $\CSym[\QAE](\qntElm)$, by applying all the
quantifier swap operations at once.
More specifically, the function $\CSym[\QEA](\cdot)$ provides a
\emph{$\QEA$-prefix}, \ie, all existential quantifier precede the universal
ones, while $\CSym[\QAE](\cdot)$ gives us the the dual \emph{$\QAE$-prefix}.

For the definition of $\CSym[\QEA](\cdot)$, we observe that every behavioral
quantifier prefix $\qntElm$ can be uniquely rewritten as $\exists^{\BSym}
\vec{\qapElm}[0] \ldotp (\forall^{\BSym} \vec{\apElm}[i] \ldotp \allowbreak
\exists^{\BSym} \vec{\qapElm}[i])_{i = 1}^{k} \ldotp \forall^{\BSym}
\vec{\apElm}[k + 1]$, for some $k \!\in\! \SetN$ and vectors $\vec{\qapElm}[i]$,
with $i \!\in\! \numcc{0}{k}$, and $\vec{\apElm}[i]$, with $i \in \numcc{1}{k +
1}$, where $\card{\vec{\qapElm}[i]}, \card{\vec{\apElm}[i]} \geq 1$, for all $i
\in \numcc{1}{k}$.
For a quantifier prefix $\qntElm$ in such a form, we then define
\vspace{-0.5em}
\[
  \CSym[\exists\forall](\qntElm) \defeq (\exists^{\BSym} \vec{\qapElm}[i])_{i =
  0}^{k} \ldotp (\forall^{\vec{\spcElm}[i]} \vec{\apElm}[i])_{i = 1}^{k + 1},
  \vspace{-0.5em}
\]
where $(\vec{\spcElm}[i])_{j} \defeq \BSym \cup \sdep{ \vec{\qapElm}[i] \cdots
\vec{\qapElm}[k] }$, for all $j \in \numco{0}{\card{\vec{\apElm}[i]}}$.

The definition of $\CSym[\QAE](\cdot)$ is analogous.
First, we rewrite a behavioral quantifier prefix $\qntElm$ as $\forall^{\BSym}
\vec{\apElm}[0] \ldotp (\exists^{\BSym} \vec{\qapElm}[i] \ldotp \forall^{\BSym}
\vec{\apElm}[i])_{i = 1}^{k} \ldotp \exists^{\BSym} \vec{\qapElm}[k + 1]$, for
some $k \!\in\! \SetN$ and vectors $\vec{\apElm}[i]$, with $i \!\in\!
\numcc{0}{k}$, and $\vec{\qapElm}[i]$, with $i \in \allowbreak \numcc{1}{k +
1}$, where $\card{\vec{\apElm}[i]}, \card{\vec{\qapElm}[i]} \!\geq\! 1$, for all
$i \!\in\! \numcc{1}{k}$.
Then, we define
\[
  \CSym[\forall\exists](\qntElm) \defeq (\forall^{\BSym} \vec{\apElm}[i])_{i =
  0}^{k} \ldotp (\exists^{\vec{\spcElm}[i]} \vec{\qapElm}[i])_{i = 1}^{k + 1},
\]
where $(\vec{\spcElm}[i])_{j} \defeq \BSym \cup \sdep{ \vec{\apElm}[i] \cdots
\vec{\apElm}[k] }$, for all $j \in \numco{0}{\card{\vec{\qapElm}[i]}}$.

\begin{example}
  \label{exm:ceacae}
  Let us consider the behavioral quantifier prefix $\qntElm = \forall^{\BSym}
  \apElm \ldotp \exists^{\BSym} \qapElm\, \rapElm \ldotp \forall^{\BSym} \sapElm
  \ldotp \exists^{\BSym} \tapElm$.
  The corresponding $\QEA$ canonical-form prefix is $\CSym[\QEA](\qntElm) =
  \exists^{\BSym} \qapElm\, \rapElm\, \tapElm \ldotp
  \forall^{\spcElm[][\apElm]}\! \apElm \ldotp \forall^{\spcElm[][\sapElm]}\!
  \sapElm$, where $\spcElm[][\apElm] \defeq \dep{\APSet}{\qapElm\, \rapElm\,
  \tapElm}$ and $\spcElm[][\sapElm] \defeq \dep{\APSet}{\tapElm}$.
  The corresponding $\QAE$ canonical-form prefix is, instead,
  $\CSym[\QAE](\qntElm) = \forall^{\BSym} \apElm\, \sapElm \ldotp
  \exists^{\spcElm} \qapElm\, \rapElm \ldotp \exists^{\BSym} \tapElm$,
  where $\spcElm \defeq \dep{\APSet}{\sapElm}$.
\end{example}

Towards the proof of the discussed equivalences, we can show the chain of
$\alpha$-implications $\CSym[\dual{\alpha}](\qntElm) \psi \cimplies[][\alpha]\,
\qntElm \psi \cimplies[][\alpha]\, \CSym[\alpha](\qntElm) \psi$ by exploiting
the following property of the $\alpha$-evolution function.
Specifically, this asserts a total ordering \wrt the preorder $\sqsubseteq$
between a behavioral quantifier prefix $\qntElm$ and its two canonical forms
$\CSym[\QEA](\qntElm)$ and $\CSym[\QAE](\qntElm)$, which can be proved by
induction.

%\defenv{proposition}[][Prp][QntSwpBas]
%  {
%  $\evlFun[\QEA](\AsgFam, \forall^{\BSym} \apElm \ldotp\!
%  \exists^{\spcElm \cup \sdep{\apElm}} \qapElm)  \!\sqsubseteq\!
%  \evlFun[\QEA](\AsgFam, \exists^{\spcElm} \qapElm \ldotp\!
%  \allowbreak \forall^{\BSym} \apElm)$ and $\evlFun[\QAE](\AsgFam,
%  \exists^{\BSym} \apElm \ldotp\!
%  \forall^{\spcElm \cup \sdep{\apElm}} \qapElm) \!\sqsubseteq\!
%  \evlFun[\QAE](\AsgFam, \forall^{\spcElm} \qapElm \ldotp\!
%  \allowbreak \exists^{\BSym} \apElm)$, for all $\AsgFam \!\in\!
%  \HAsgSet(\PSet)$ with $\PSet \!\subseteq\! \APSet$, $\apElm, \qapElm \in
%  \APSet \setminus \PSet$, and $\spcElm \in \SpcSet[\BSym]$.
%  }

\defenv{proposition}[][Prp][QntSwpInd]
  {
  $\!\evlFun[\alpha](\AsgFam, \CSym[\dual{\alpha}](\qntElm)) \!\sqsubseteq\!
  \evlFun[\alpha](\AsgFam, \qntElm) \!\sqsubseteq\! \evlFun[\alpha](\AsgFam,
  \CSym[\alpha](\qntElm))$, for all $\AsgFam \in \HAsgSet$ and $\qntElm \in
  \QntSet[\BSym]$, with $\ap{\qntElm} \cap \ap{\AsgFam} = \emptyset$.
  }

%\defenv{proposition}[][Prp][QntSwpIndI]
%  {
%  $\!\evlFun[\alpha](\AsgFam, \CSym[\dual{\alpha}](\qntElm[1] \ldotp
%  \qntElm[2])) \!\sqsubseteq\! \YFam \!\sqsubseteq\! \evlFun[\alpha](\AsgFam,
%  \qntElm[1] \ldotp \qntElm[2])$, for all $\YFam \in \{
%  \evlFun[\alpha](\AsgFam, \qntElm[1] \ldotp \CSym[\dual{\alpha}](\qntElm[2])),
%  \evlFun[\alpha](\AsgFam, \CSym[\dual{\alpha}](\qntElm[1]) \ldotp \qntElm[2])
%  \}$, $\AsgFam \in \HAsgSet$ and $\qntElm[1], \qntElm[2] \in \QntSet[\BSym]$,
%  with $\ap{\qntElm[1] \ldotp \qntElm[2]} \cap \ap{\AsgFam} = \emptyset$.
%  }

%\defenv{proposition}[][Prp][QntSwpIndII]
%  {
%  $\!\evlFun[\alpha](\AsgFam, \qntElm[1] \ldotp \qntElm[2]) \!\sqsubseteq\!
%  \YFam \!\sqsubseteq\! \evlFun[\alpha](\AsgFam, \CSym[\alpha](\qntElm[1]
%  \ldotp \qntElm[2]))$, for all $\YFam \in \{ \evlFun[\alpha](\AsgFam,
%  \qntElm[1] \ldotp \CSym[\alpha](\qntElm[2])), \evlFun[\alpha](\AsgFam,
%  \CSym[\alpha](\qntElm[1]) \ldotp \qntElm[2]) \}$, $\AsgFam \in \HAsgSet$ and
%  $\qntElm[1], \qntElm[2] \in \QntSet[\BSym]$, with $\ap{\qntElm[1] \ldotp
%  \qntElm[2]} \cap \ap{\AsgFam} = \emptyset$.
%  }


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Article"
%%% End:


==> SectionIIIb.tex <==

\subsection{Quantification Game for Sentences}

The following result establishes the equisatisfiability of any behavioral
\GFG-\QPTL sentence \wrt both its canonical form.

\defenv{theorem}[Sentence Canonical Forms][Thm][SntCanFor]
  {
  For every behavioral \GFG-\QPTL sentence $\qntElm \psi$, with $\psi \in \LTL$,
  it holds that $\qntElm \psi$, $\CSym[\QEA](\qntElm) \psi$, and
  $\CSym[\QAE](\qntElm) \psi$ are equisatisfiable.
  }

The proof of Theorem~\ref{thm:sntcanfor} can be split in two parts.
The first one shows the implication chain $\CSym[\dual{\alpha}](\qntElm) \psi
\cimplies[][\alpha]\, \qntElm \psi \cimplies[][\alpha]\, \CSym[\alpha](\qntElm)
\psi$ using Proposition~\ref{prp:qntswpind} by logically concatenating it with
Lemma~\ref{lmm:prfevl} and Theorem~\ref{thm:hypref}.
For the second part, we are now left with showing that $\CSym[\alpha](\qntElm)
\psi \cimplies[][\alpha]\, \CSym[\dual{\alpha}](\qntElm) \psi$.
Unfortunately, this cannot be derived from the $\sqsubseteq$-based inclusion
between the $\alpha$-evolutions of $\CSym[\alpha](\qntElm)$ and
$\CSym[\dual{\alpha}](\qntElm)$.
If this were the case, indeed, we would obtain the determinacy of arbitrary
$\omega$-round games, which is known to be false~\cite{GS53}.
Driven by this connection, the proof follows a game-theoretic argument, which
explicitly exploits the $\omega$-regularity of \LTL languages and, in
particular, their membership in the Borelian hierarchy of the Cantor topological
space of infinite words~\cite{PP04}.

To define the quantification game, we first need a few notions.
%
A two-player turn-based \emph{arena} $\Arena = \tuple {\PPosSet} {\OPosSet}
{\iposElm} {\MovRel}$ is a tuple where
\begin{inparaenum}
  \item
    $\PPosSet$ and $\OPosSet$ are the sets of \emph{positions} of \emph{Eloise}
    and \emph{Abelard}, \aka \emph{Player} and \emph{Opponent}, respectively,
    with $\PPosSet \cap \OPosSet = \emptyset$,
  \item
    $\iposElm \in \PosSet \defeq \PPosSet \cup \OPosSet$ is the \emph{initial
    position}, and
  \item
    $\MovRel \subseteq \PosSet \times \PosSet$ is the binary relation describing
    all possible \emph{moves} such that $\tuple{\PosSet}{\MovRel}$ is a sinkless
    directed graph.
\end{inparaenum}
%
A \emph{game} $\Game = \tuple {\Arena} {\ObsSet} {\WinSet}$ is a tuple where
$\Arena$ is an arena, $\ObsSet \subseteq \PosSet$ is the set of \emph{observable
positions}, and $\WinSet \subseteq \ObsSet^{\omega}$ is the set of
\emph{observable sequences} that are \emph{winning} for Eloise; the complement
$\dual{\WinSet} \defeq \ObsSet^{\omega} \setminus \WinSet$ is \emph{winning} for
Abelard.
%
Eloise (\resp, Abelard) \emph{wins} the game if she (\resp, he) has a strategy
such that, for all adversary strategies, the corresponding play induces an
observation sequence belonging (\resp, not belonging) to $\WinSet$.
All notions necessary to formalize this intuition, as \emph{history},
\emph{strategy}, and \emph{play}, are given in Appendix~\ref{app:canqnt}.\!

Martin's determinacy theorem~\cite{Mar75,Mar85} states that all Borelian games
are determined, \ie, when the winning condition $\WinSet$ is a Borel set, either
one of the two players necessarily wins the game.
To ensures that the quantification game we are about to define is indeed
determined, we require a form of Borelian condition that can be applied to sets
of assignments.
This determinacy requirement is crucial here, since it is tightly connected with
the fact that \GFG-\QPTL does not allow for undetermined formulae.
%
To this end, let $\ValSet \defeq \APSet \pto \SetB$ denote the set of Boolean
valuations for (sub)sets of propositions and $\ValSet(\PSet) \defeq \set{
\valElm \in \ValSet }{ \dom{\valElm} = \PSet }$ the set of valuations for
propositions in $\PSet \!\subseteq\! \APSet$.
Also, $\#(\valElm) \defeq \card{\dom{\valElm}}$.
%
We can now define a bijection between sets of assignments and languages of
infinite words over the alphabet $\ValSet(\PSet)$ as follows.
Let $\SetNI \defeq \SetN \cup \{ \omega \}$ and $\ValSet(\PSet)^{\infty} \defeq
\ValSet(\PSet)^{*} \cup \ValSet(\PSet)^{\omega}$.
Moreover, let $\wrdFun \colon \AsgSet(\PSet) \times \SetNI \to
\ValSet(\PSet)^{\infty}$ be the \emph{word function} mapping each assignment
$\asgElm \in \AsgSet(\PSet)$ and number $k \in \SetNI$ to the word $\wrdElm
\defeq \wrdFun(\asgElm, k) \in \ValSet(\PSet)^{k}$ of length $k$ on the alphabet
$\ValSet(\PSet)$ satisfying the equality $\asgElm(\apElm)(t) =
(\wrdElm)_{t}(\apElm)$, for all $\apElm \in \PSet$ and $t \in \numco{0}{k}$.
Then, the induced function $\wrdFun(\cdot) \defeq \allowbreak \wrdFun(\cdot,
\omega) \colon \AsgSet(\PSet) \to \ValSet(\PSet)^{\omega}$ with the second
argument fixed to $\omega$ is clearly a bijection.
%
Every property $\Psi \subseteq \AsgSet(\PSet)$, \ie, every set of assignments,
uniquely induces the language of infinite words $\WSet(\Psi) \defeq \set{
\wrdFun(\asgElm) }{ \asgElm \in \Psi } \subseteq \ValSet(\PSet)^{\omega}$ over
the alphabet $\ValSet(\PSet)$.
Thus, $\Psi$ is said to be \emph{Borelian} (\resp, regular) if the language
$\WSet(\Psi)$ is a Borel (\resp, regular) set.

\begin{figure}[htbp]
  \vspace{-0.5em}
  \begin{center}
    \scalebox{0.85}[0.65]{\figqntgam}
  \end{center}
  \vspace{-1em}
  \caption{\label{fig:gntgam} Quantification game for $\qntElm = \exists^{\BSym}
  \apElm[1] \ldotp \forall^{\BSym} \apElm[2]\ldotp \exists^{\BSym} \apElm[3]
  \cdots$. Eloise owns the circled positions, while Abelard the squared ones.
  From the total-valuation positions $\valElm[1], \ldots, \valElm[n]$, with $n =
  \pow{\card{\ap{\qntElm}}}$, Abelard moves to the initial position.}
  \vspace{-0.5em}
\end{figure}

Given a behavioral sentence $\varphi \defeq \qntElm \psi$, let $\Psi$ denote the
set of assignments satisfying the \LTL formula $\psi$.
The quantification game $\Game[\qntElm][\Psi]$ for $\varphi$ is defined in
Construction~\ref{cns:qntgami} and exemplified in Figure~\ref{fig:gntgam}.
\Wlogx, we assume that the prefix $\qntElm$ does not contain duplicates.
The positions of the game are (partial) valuations of the propositions in the
prefix $\qntElm$ and each position belongs to the player corresponding to the
first quantifier in the prefix $\qntElm$ whose proposition is not defined at
that position.
The initial position of the game contains the empty valuation and in the example
of Figure~\ref{fig:gntgam} belongs to Eloise, she being the first to play in
$\qntElm$.
Obviously, the game features an infinite number of rounds.
Each round begins with the empty valuation and ends in a total valuation, after
both players have chosen a value for all the propositions.
A move in the round corresponds to a player choosing a value for the next
proposition in the prefix.
Take, for instance, position $\valElm \defeq \{ \apElm[1] \mapsto \Ff \}$ in the
figure, where the first proposition $\apElm[1]$ has been already assigned value
$\Ff$ by Eloise.
From that position, Abelard first chooses a Boolean value, say $\Tt$, for the
next proposition $\apElm[2]$ in the prefix.
Then he moves to the position $\valElm' \defeq \{ \apElm[1] \mapsto \Ff,
\apElm[2] \mapsto \Tt \}$, corresponding to the valuation ${\valElm}[\apElm[2]
\mapsto \Tt]$, obtained by extending $\valElm$ with the value chosen for
$\apElm[2]$.
Position $\valElm'$ belongs to Eloise, since the next quantifier $\exists
\apElm[3]$ in the prefix is existential.
The last position belongs to Abelard and, from there, he can only move back to
the starting position for the next turn.
%
By sampling any infinite sequence of rounds of the games at the positions with
total valuations, namely the observable positions, we obtain an infinite word
$\wrdElm$ corresponding to some assignment $\asgElm \defeq
\wrdFun[][-1](\wrdElm)$.
Then, $\wrdElm$ is winning for Eloise \iff $\asgElm$ belongs to $\Psi$ (\ie,
$\asgElm \models \psi$), while it is winning for Abelard otherwise.
This intuition is formalized by the following construction.

\begin{construction}[Quantification Game I]
  \label{cns:qntgami}
  For every quantifier prefix $\qntElm \in \QntSet[\BSym]$ and property $\Psi
  \subseteq \AsgSet(\ap{\qntElm})$, the game $\Game[\qntElm][\Psi] \defeq
  \allowbreak \tuple {\Arena[\qntElm]} {\ObsSet} {\WinSet}$ with arena
  $\Arena[\qntElm] \defeq \tuple {\PPosSet} {\OPosSet} {\iposElm} {\MovRel}$ is
  defined as prescribed in the following:
  \begin{itemize}
    \item
      the set of positions $\PosSet \subset \ValSet$ contains exactly those
      valuations $\valElm \in \ValSet$ of the propositions in $\ap{\qntElm}$
      that are quantified in the prefix $(\qntElm)_{< \#(\valElm)}$ of $\qntElm$
      having length $\#(\valElm)$ \ie, $\dom{\valElm} = \ap{(\qntElm)_{<
      \#(\valElm)}}$;
    \item
      the set of Eloise's positions $\PPosSet \subseteq \PosSet$ only contains
      the valuations $\valElm \in \PosSet$ for which the proposition quantified
      in $\qntElm$ at index $\#(\valElm)$ is existentially quantified, \ie,
      $(\qntElm)_{\#(\valElm)} = \exists^{\BSym} \apElm$, for some $\apElm \in
      \ap{\qntElm}$;
    \item
      the initial position $\iposElm \defeq \emptyfun$ is just the empty
      valuation;
    \item
      the move relation $\MovRel \subseteq \PosSet \times \PosSet$ contains
      exactly those pairs of valuations $(\valElm[1], \valElm[2]) \in \PosSet
      \times \PosSet$ such that:
      \begin{itemize}
        \item
          $\valElm[1] \subseteq \valElm[2]$ and $\#(\valElm[2]) = \#(\valElm[1])
          + 1$;
        \item
          $\valElm[1] \in \ValSet(\ap{\qntElm})$ and $\valElm[2] = \emptyfun$;
      \end{itemize}
    \item
      the set of observable positions $\ObsSet \defeq \ValSet(\ap{\qntElm})$
      precisely contains the valuations of all the propositions in $\qntElm$;
    \item
      the winning condition induced by the property $\Psi$ is the language of
      infinite words $\WinSet \defeq \WSet(\Psi)$ over $\ValSet(\ap{\qntElm})$.
  \end{itemize}
\end{construction}

Clearly, the game $\Game[\qntElm][\Psi]$ just described formalizes the intuitive
game-theoretic argument used to justify the quantifier swap of the previous
subsection.
By exploiting the following interpretation of the $\QEA$-evolution of the two
canonical-forms in game-theoretic terms, we can finally prove that $\qntElm
\psi$ is indeed equivalent to both $\CSym[\QAE](\qntElm) \psi$ and
$\CSym[\QEA](\qntElm) \psi$.

\defenv{theorem}[Quantification Game I][Thm][QntGamI]
  {
  For each behavioral quantification prefix $\qntElm \!\in\! \QntSet[\BSym]$ and
  Borelian property $\!\Psi \!\subseteq\! \AsgSet(\ap{\qntElm})$,\! the game
  $\Game[\qntElm][\Psi]$ satisfies the following two properties:
  \begin{enumerate}[1)]
    \item\labelx{elo}
      if Eloise wins then $\ESet \subseteq \Psi$, for some $\ESet \in
      \evlFun[\QEA](\CSym[\QAE](\qntElm))$;
    \item\labelx{abe}
      if Abelard wins then $\ESet \not\subseteq \Psi$, for all $\ESet \in
      \evlFun[\QEA](\CSym[\QEA](\qntElm))$.
  \end{enumerate}
  }

The idea of the proof is to extract, from a winning strategy of Eloise
(\resp, Abelard), a vector $\vec{\FFun}$ of functors, one for each proposition
associated with that player, witnessing the existence (\resp, non-existence) of
a set $\ESet$ of assignments satisfying the property $\Psi$.
More precisely, assume Eloise has a strategy $\strElm$ to win the game and let
$\forall^{\BSym} \vec{\apElm} \ldotp \exists^{\vec{\spcElm}} \vec{\qapElm} =
\CSym[\QAE](\qntElm)$ be the $\QAE$ canonical-form of $\qntElm$.
Then, thanks to the bijection between plays $\playElm$ and assignments
$\asgElm$, we can operate as follows, for every round $k$ and existential
proposition $\qapElm[i]$ in $\vec{\qapElm}$: given Abelard's choices up to round
$k$ in $\playElm$, we can extract, from Eloise's response for $\qapElm[i]$ in
$\strElm$, the response to $\asgElm$ at time $k$ of the functor $\FFun[i]$ in
$\vec{\FFun}$.
As a consequence, for all $\asgElm \in \AsgSet(\vec{\apElm})$ chosen by Abelard,
Eloise's response corresponding to the extension of $\asgElm$ with $\vec{\FFun}$
on $\vec{\qapElm}$ satisfies, \ie, belongs to, the property $\Psi$.
The witness $\ESet$ is precisely the set of all those extensions.
An analogous argument applies to Abelard for the $\QEA$ canonical-form.

We can now complete the proof of Theorem~\ref{thm:sntcanfor}, by focusing on
the implication $\CSym[\QEA](\qntElm) \psi \cimplies[][\QEA]\,
\CSym[\QAE](\qntElm) \psi$, since the dual one $\CSym[\QAE](\qntElm) \psi
\cimplies[][\QAE]\, \CSym[\QEA](\qntElm) \psi$ can be derived by means of
Theorem~\ref{thm:dlt}.
%
Thanks to Lemma~\ref{lmm:prfevl}, if $\{\!\{ \emptyfun \}\!\} \cmodels[][\QEA]
\CSym[\QEA](\qntElm) \psi$, then $\ESet \subseteq \Psi$, for some $\ESet \in
\evlFun[\QEA](\CSym[\QEA](\qntElm))$.
Thus, by Item~\ref{thm:qntgami(abe)} of Theorem~\ref{thm:qntgami}, it follows
that Abelard loses the game $\Game[\qntElm][\Psi]$, which means, by determinacy,
that Eloise wins.
As a consequence of Item~\ref{thm:qntgami(elo)} of the same theorem, there
exists $\ESet \in \evlFun[\QEA](\CSym[\QAE](\qntElm))$ such that $\ESet
\subseteq \Psi$.
Hence, $\{\!\{ \emptyfun \}\!\} \cmodels[][\QEA] \CSym[\QAE](\qntElm) \psi$,
again by Lemma~\ref{lmm:prfevl}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Article"
%%% End:


==> SectionV.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% SectionV.tex                                                               %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 2020, Dylan Bellier, Massimo Benerecetti, Dario Della Monica,%%
%%                     and Fabio Mogavero.                                    %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file SectionV.tex

\section{Expressiveness \& Succinctness}
\label{sec:expsuc}

\cbstart
...
\cbend

\begin{theorem}[Vanilla to Behavioral]
  \label{thm:vanbhv}
  For every \QPTL formula, there exists an equivalent behavioral \QPTL one.
\end{theorem}

\cbstart
...
\cbend

\begin{theorem}[Behavioral to Vanilla]
  \label{thm:bhvvan}
  For every behavioral \QPTL formula, there exists an equivalent \QPTL one.
\end{theorem}

\cbstart
...
\cbend

\begin{theorem}[Succinctness]
  \label{thm:suc}
  \QPTL is non-elementary more succinct than behavioral \QPTL.
\end{theorem}

% End of file SectionV.tex


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Article"
%%% End:


==> SectionVI.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% SectionVI.tex                                                              %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file SectionVI.tex

\begin{section}{...}
  \label{sec:vi}

  \cbstart
  ...
  \cbend


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}

\end{section}

% End of file SectionVI.tex


==> SectionVII.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% SectionVII.tex                                                             %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file SectionVII.tex

\begin{section}{...}
  \label{sec:vii}

  \cbstart
  ...
  \cbend


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}

\end{section}

% End of file SectionVII.tex


==> SectionVIII.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% SectionVIII.tex                                                            %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file SectionVIII.tex

\begin{section}{...}
  \label{sec:viii}

  \cbstart
  ...
  \cbend


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}


  \begin{subsubsection}{...}

    \cbstart
    ...
    \cbend

  \end{subsubsection}

\end{section}

% End of file SectionVIII.tex


==> Tables.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Tables.tex                                                                 %%
%%                                                                            %%
%% Revision 0                                                                 %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Tables.tex

%%****************************************************************************%%
%% Required packages                                                          %%
%%****************************************************************************%%

\usepackage{multirow}

%%****************************************************************************%%

%%****************************************************************************%%
%% Basic settings                                                             %%
%%****************************************************************************%%

% ...

%%****************************************************************************%%

%%****************************************************************************%%
%% Tables                                                                     %%
%%****************************************************************************%%

\AfterEndPreamble
  {

  %%**************************************************************************%%

  \newcommand{\tab}
    {
    \begin{wraptable}[5]{r}{0.200\textwidth}
      \vspace{-1em}
      \begin{center}
        \small
        \scalebox{1.00}[1.00]
          {
          \begin{tabular}{}
          \end{tabular}
          }
        \caption{\label{tab:...} \small ... .}
      \end{center}
      \vspace{-1em}
    \end{wraptable}
    }

  %%**************************************************************************%%

  }

%%****************************************************************************%%

% End of file Tables.tex

